UniIntervene++: An Adaptive Intervention Agent for Efficient Real-World Reinforcement Learning

Online reinforcement learning (RL) enables robot policies to improve through physical interaction, but the assistance they require changes as their competence evolves. Existing intervention strategies based on offline estimates or fixed decision rules can therefore become mismatched to the current policy. To address this, we propose UniIntervene++, an adaptive intervention agent that learns to allocate control between autonomous execution and heterogeneous assisted behaviors during online RL. Specifically, UniIntervene++ first formulates the evolving RL policy, trajectory correction, and a task-structured CodePolicy as Options in a unified semi-Markov decision process and learns their relative values online. Building on this, competence-adaptive intervention periodically probes the RL policy through unassisted execution, keeping control allocation responsive to its evolving capability. Finally, coupled experience learning allows assisted behaviors to improve the RL policy, whose evolving outcomes in turn reshape future intervention decisions. In this way, UniIntervene++ jointly determines when to intervene, how to intervene, and when to return control as the RL policy improves. Across five real-world manipulation tasks, UniIntervene++ achieves an average success rate of 89.67%, outperforming all baselines by at least 6 percentage points, while reducing human intervention to 0.77%, a relative reduction of at least 94.6% from the best baseline. Code is available in our \href{https://github.com/dannyyudong/An-Adaptive-Intervention-Agent-for-Efficient-Real-World-Reinforcement-Learning}{GitHub repository}.

==> table/results_table_1.tex <==
% Publication-ready grouped three-line table.
% Requires booktabs, makecell, and multirow.
% The first success fraction in each source cell is used as SR.
% Secondary checkpoint entries are intentionally omitted pending clarification:
% HIL-SERL/Tube: 4/10 = 40%; HIL-SERL/USB: 42/60 = 70%;
% AutoSERL/Board: 17/60 = 28.3% (or 41.7% if "+8" means 8 successes).
% AutoSERL/Tube IR=0.24 is treated as a fraction and shown as 24.0%.
% AutoSERL/Tube HIR=0.001 is treated as a fraction and shown as 0.10%.
\begin{table*}[t]
    \caption{Real-world manipulation results across five tasks spanning
pick-and-place, contact-rich manipulation, and deformable-object manipulation. Bold numbers
denote the best result for each task and metric.}
    \label{tab:task-results}
    \centering
    \begingroup
    \footnotesize
    \setlength{\tabcolsep}{0.8pt}
    \renewcommand{\arraystretch}{1.16}
    \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}l*{18}{c}@{}}
        \toprule
        \multirow{3}{*}{\textbf{Method}}
        & \multicolumn{3}{c}{\textbf{Pick-and-place}}
        & \multicolumn{9}{c}{\textbf{Contact-rich}}
        & \multicolumn{3}{c}{\textbf{Deformable-Object}}
        & \multicolumn{3}{c}{\textbf{Average}} \\
        \cmidrule(lr){2-4}\cmidrule(lr){5-13}\cmidrule(lr){14-16}
        & \multicolumn{3}{c}{Ring Transfer}
        & \multicolumn{3}{c}{\makecell[c]{Tube  Insertion}}
        & \multicolumn{3}{c}{\makecell[c]{USB  Insertion}}
        & \multicolumn{3}{c}{\makecell[c]{Whiteboard  Wipe}}
        & \multicolumn{3}{c}{\makecell[c]{Towel  Folding}}
        & \multicolumn{3}{c}{} \\
        \cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
        \cmidrule(lr){11-13}\cmidrule(lr){14-16}
        & SR$\uparrow$ & IR$\downarrow$ & HIR$\downarrow$
        & SR$\uparrow$ & IR$\downarrow$ & HIR$\downarrow$
        & SR$\uparrow$ & IR$\downarrow$ & HIR$\downarrow$
        & SR$\uparrow$ & IR$\downarrow$ & HIR$\downarrow$
        & SR$\uparrow$ & IR$\downarrow$ & HIR$\downarrow$
        & SR$\uparrow$ & IR$\downarrow$ & HIR$\downarrow$ \\
        \midrule
        HIL-SERL
        & 83.33 & 39.15 & 39.15
        & 85 & 39.65 & 39.65
        & 90 & 51.68 & 51.68
        & 85 & 63.11 & 63.11
        & 75 & 76.57 & 76.57
        & 83.67 & 54.03 & 54.03 \\
        AutoSERL
        & 53.33 & 46.37 & 17.07
        & 80 & \textbf{24.0} & \textbf{0.10}
        & 88.3 & 41.11 & 3.91
        & 80 & \textbf{41.23} & 16.80
        & 66.67 & \textbf{58.89} & 33.55
        & 73.66 & \textbf{42.32} & 14.29 \\
        UniIntervene
        & 85 & \textbf{36.62} & 25.32
        & 73.33 & 49.1 & 15.8
        & 90 & \textbf{20.14} & 9.9
        & \textbf{90} & 58.3 & 10.9
        & 80 & 64.3 & 32.3
        & 83.67 & 45.69 & 18.84 \\
        \midrule
        \textbf{UniIntervene++}
        & \textbf{88.33} & 45.76  & \textbf{0.3}
        & \textbf{91.6} & 58.89 & 2.58
        & \textbf{96.67} &52.48 & \textbf{0.96}
        & 86.67 & 60 & \textbf{0.01}
        & \textbf{85} & 63.08 & \textbf{0}
        & \textbf{89.65} & 56.04 & \textbf{0.77} \\
        \bottomrule
    \end{tabular*}
    \endgroup
\end{table*}


==> table/training_time_table.tex <==
% Single-column training-time table for the five real-robot tasks.
% Requires booktabs and makecell (loaded in root.tex).
\begin{table}[t]
    \caption{Training Time Across 5 Real-Robot Tasks}
    \label{tab:training-time}
    \centering
    \begingroup
    \footnotesize
    \setlength{\tabcolsep}{2pt}
    \renewcommand{\arraystretch}{1.15}
    \begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}}lcc@{}}
        \toprule
        \textbf{Task}
        & \textbf{Training step}
        & \textbf{Training Time (min)} \\
        \midrule
        Towel Folding
        & 32,000
        & 52 \\
        Ring Transfer
        & 82,000
        & 131 \\
        Tube Insertion
        & 40,000
        & 64 \\
        USB Insertion
        & 18,000
        & 29 \\
        Wipe Whiteboard
        & 68,000
        & 105 \\
        \bottomrule
    \end{tabular*}
    \endgroup
\end{table}

